Learning with Instance Bundles for Reading Comprehension

When training most modern reading comprehension models, all the questions associated with a context are treated as being independent from each other. However, closely related questions and their corresponding answers are not independent, and leveraging these relationships could provide a strong supervision signal to a model. Drawing on ideas from contrastive estimation, we introduce several new supervision techniques that compare question-answer scores across multiple related instances. Specifically, we normalize these scores across various neighborhoods of closely contrasting questions and/or answers, adding another cross entropy loss term that is used in addition to traditional maximum likelihood estimation. Our techniques require bundles of related question-answer pairs, which we can either mine from within existing data or create using various automated heuristics. We empirically demonstrate the effectiveness of training with instance bundles on two datasets -- HotpotQA and ROPES -- showing up to 11% absolute gains in accuracy.

==> ACL2021/2-6-comp-function.tex <==
\subsection{Compatibility Function}
\label{sec:scores}
The compatibility function is dependent on the design of the base question answering model. Here we will discuss some of the plausible ways to define compatibility function, $\psi$, for modeling different answer output spaces.

In a \textbf{multi-choice} QA setup~\cite{lai2017race}, it can be log-likelihood of a given target answer over a fixed set of answer candidates, similar to cross-entropy loss.

In a \textbf{span selection}~\cite{chen2017reading} model, it can be the likelihood of answer span computed by summing log-probablity of all the tokens in the span.

In a \textbf{BIO tagging} model~\cite{segal2019simple} it can be the probability of an answer span which is summation of log-probabilities of ``B" tag for the first and ``I" tag for the remaining tokens in a span. 

In an \textbf{Encoder-Decoder} style answer generation  model~\cite{raffel2019exploring}, a simple compatibility function entails summing up log-probabilities of each token in the span. We focus on this style of answering model in our experiments and will elaborate more on this in Section~\ref{sec:gen_score}.

In all our formulations, we assume compatibility function return an exponentiated score, $\psi(\cdot) = \exp f (\cdot)$. The compatibility scores can be normalized over different combinations of neighborhoods which allow for different probabilistic interpretations.

==> ACL2021/4-2-comp-gen.tex <==
\subsection{Compatabiliy functions for conditional generation models}
\label{sec:gen_score}
To understand the role of compatibility functions, we experiment with a few choices of compatibility functions. We first present those alternatives, and then show results of experiments with them. Our choice of compatibility functions are specific to encoder-decoder style architecture. 

A transformer style decoder, $d$, can be described as a markov random field~\cite{deng2020cascaded} which takes as input previous answer tokens and question to output current answer token at time step, $t$, as shown in Figure~\ref{fig:answer_decode_graph}. This decoder allows for independent parallel prediction of tokens at each time step, which make the answer likelihood a product of independent markov random fields,  $\prod_t p(a_t|a_{<t},q)$, tied by same parameters in function $d$.

% \matt{I don't think you need the above discussion at all.  You just say that given a candidate answer and a question, the model produces a score.  Basically all models can be viewed this way, and we focus on generative QA models, using T5 in particular in our experiments.
% The discussion below should be moved somewhere else, I think, as I recommended above.  It's a relatively small point about how to do scoring in generative models, and how that interacts with CE, and it's distracting to have it before the main contribution.}


\begin{figure}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{observed}=[circle,draw,fill=lightgray,text=black,minimum size=1.2cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1.2cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1.2cm]

  \node[latent]           (A)                  {$a_t$};
  \node[observed]         (B) [below of=A]     {$a_{t-1}$};
  \node[ellipsis]         (C) [left of=B, xshift=0.6cm]      {\ldots};
  \node[observed]         (D) [left of=C, xshift=0.6cm]      {$a_1$};
  \node[observed]         (E) [left of=D, xshift=-0.4cm]      {$a_0$};
  
  \path (A) edge              node {} (B)
            edge              node {} (D)
            edge              node {} (E);
       
\end{tikzpicture}
\caption{Answer decoder}
\label{fig:answer_decode_graph}
\end{figure}

\paragraph{Locally-normalized (LN)} scores can be defined as sum of log-probability of token at each time step locally normalized over vocabulary.
\begin{equation*}
    \begin{split}
         \psi_L(q,a) &= \exp \log \prod_t p(a_t|a_{<t}, q)  \\
         &= \exp \sum_{t} \log \frac{\exp(d(a_t; a_{<t},q))}{\sum_{v \in |V|} \exp(d(v; a_{<t},q))}
    \end{split}
\end{equation*}



\paragraph{Un-normalized scores (UN):}
Locally normalized scores may suffer from label bias~\cite{goyal2019empirical} which can be crucial when contrastive answers that have overlapping subsequences, for eg., if answer candidates are a list of choices \{``Person A", ``Person B", ``Person C"\}. 

\begin{equation*}
    \begin{split}
         \psi_U(q,a) &= 
         \exp \log \prod_{t} \exp(d(a_t; a_{<t},q)) \\
         &= \exp \log \exp(\sum_{t} d(a_t; a_{<t},q)) \\
         &  = \exp \sum_{t} d(a_t; a_{<t},q)
    \end{split}
\end{equation*}


\paragraph{ Whole Sequence (GS):} score considers the score of the last token, which is often a special symbol like, $\langle eos \rangle$ tag. Intuitively, this can be seen as a score for the entire input answer sequence, $\psi_G(q, a) = d(a_T; a_{<T},q)$


\subsubsection{Ablation results}
From Table~\ref{tab:comp_results} and Table~\ref{tab:ropes_results} we can see that the question conditional loss overall works well. Interestingly GS compatibility function performs well on COMPARISON but not on ROPES. We conjecture that's because in ROPES often the candidates have very small lexical dissimilarities (e.g., ``Patient A", ``Patient B") which makes looking at each token important. In ROPES, full partition loss performs slightly better than question conditions. 

\begin{table*}[!htp]
\centering
    \small
    \begin{tabular}{lccccc}
    \toprule
       & \multicolumn{2}{c}{\textbf{Single Neighborhood}} & \multicolumn{3}{c} {\textbf{Multiple Neighborhood}} \\
    \cmidrule(lr){2-3}  \cmidrule(lr){4-6} 
    &   {Answer Conditional} & {Question Conditional} & {Two-way} &   {Joint} & {Full Partition} \\
     \midrule
      \textbf{LN}  & 76.0/83.7 & \textbf{77.4/84.7} & 75.5/82.7  &  75.6/83.1 & 73.2/81.1  \\
      \textbf{UN}  & 75.7/82.9 & 76.6/84.6 & 75.3/82.6 & 75.6/83.3 & 76.7/84.7 \\ 
      \textbf{GS} & 76.9/84.1 & 76.4/83.6 & 76.0/83.2 &  74.7/81.5 & 75.7/83.3\\
    \bottomrule
    \end{tabular}
    \caption{Performance (EM/F1) of COMPARISON dev set on models finetuned with different single and multiple neighborhood CE losses.}
    \label{tab:comp_results}
\end{table*}
\begin{table*}[!htp]
\centering
    \small
    \begin{tabular}{lccccc}
    \toprule
       & \multicolumn{2}{c}{\textbf{Single Neighborhood}} & \multicolumn{3}{c} {\textbf{Multiple Neighborhood}} \\
    \cmidrule(lr){2-3}  \cmidrule(lr){4-6} 
    &   {Answer Conditional} & {Question Conditional} & {Two-way}  & {Joint}  & {Full Partition} \\
     \midrule
      \textbf{LN}  &  74.5 & 76.6 & 73.5  &  72.5 & 75.1\\
      \textbf{UN}  & 73.0 & 75.9 & 74.9  &  71.2 &  \textbf{77.6}\\
      \textbf{GS}  & 71.8 & 69.5 & 71.1 & 69.7 & 73.1\\
    \bottomrule
    \end{tabular}
    \caption{Performance (EM) of ROPES dev set on models finetuned with different single and multiple neighborhood CE losses. We do not report F1 as it's not a good performance measure on this dataset}
    \label{tab:ropes_results}
\end{table*}


% \begin{table*}[!htp]
% \centering
%     \small
%     \begin{tabular}{lcccccc}
%     \toprule
%       & \multicolumn{2}{c}{\textbf{Single Neighborhood}} & \multicolumn{4}{c} {\textbf{Multiple Neighborhood}} \\
%     \cmidrule(lr){2-3}  \cmidrule(lr){4-7} 
%     &   {Answer Conditional} & {Question Conditional} & {Two-way} &  {Multi-label}  & {Joint} & {Full Partition} \\
%      \midrule
%       \textbf{LN}  & 76.0/83.7 & \textbf{77.4/84.7} & 75.5/82.7  & 74.0/80.7 & 75.6/83.1 & 73.2/81.1  \\
%       \textbf{UN}  & 75.7/82.9 & 76.6/84.6 & 75.3/82.6 & 76.0/84.1 & 75.6/83.3 & 76.7/84.7 \\ 
%       \textbf{GS} & 76.9/84.1 & 76.4/83.6 & 76.0/83.2 &  75.6/82.7 & 74.7/81.5 & 75.7/83.3\\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison EM/F1 contrastive estimation}
%     \label{tab:comp_results}
% \end{table*}
% \begin{table*}[!htp]
% \centering
%     \small
%     \begin{tabular}{lcccccc}
%     \toprule
%       & \multicolumn{2}{c}{\textbf{Single Neighborhood}} & \multicolumn{4}{c} {\textbf{Multiple Neighborhood}} \\
%     \cmidrule(lr){2-3}  \cmidrule(lr){4-7} 
%     &   {Answer Conditional} & {Question Conditional} & {Two-way}  & {Multi-label}  & {Joint}  & {Full Partition} \\
%      \midrule
%       \textbf{LN}  &  74.5 & 76.6 & 73.5  & 69.4 & 72.5 & 75.1\\
%       \textbf{UN}  & 73.0 & 75.9 & 74.9  & 70.2 & 71.2 &  \textbf{77.6}\\
%       \textbf{GS}  & 71.8 & 69.5 & 71.1 & 70.6 & & 73.1\\
%     \bottomrule
%     \end{tabular}
%     \caption{ROPES EM contrastive estimation}
%     \label{tab:ropes_results}
% \end{table*}


==> ACL2021/old_versions/2-background.tex <==
\section{Background}
\label{sec:setup_old}

Given a training instance bundle of related question-answer pairs, $\mathcal{B} = \{(q_0...q_n),(a_0...a_n)\}$, the goal is to learn a probabilistic model that maximizes the joint likelihood of aligning the correct question and answer pairs in an instance bundle. 
\subsection{Instance bundles}
As shown in Figure~\ref{fig:hotpot_ex_bundle}, instance bundles are a group of related questions with a necessary constraint that there is an injective mapping between the question and answer space, i.e., only a single item from answer space can be matched to an item in the question space and vice-versa. For a given answer $a_i$ in all possible answer candidates $\mathcal{A}$, we define a neighbourhood around $a_i$, as $\{a_1,..a_{i-1},a_{i+1},..a_n\} = \mathcal{A}_{\mathcal{B}} \setminus a_i$  and $q_i$, as $\{q_1,..q_{i-1},q_{i+1},..q_n\} = \mathcal{Q}_{\mathcal{B}} \setminus q_i $. We present several probabilistic models that learn the dependencies between  $\mathcal{A}_{\mathcal{B}}$ and $\mathcal{Q}_{\mathcal{B}}$ contrastively.
We assume that the neighborhood exclusively contains negative samples, i.e. $\forall (a_i, a_k) \in \{\mathcal{A}_{\mathcal{B}}\} \times \{\mathcal{A}_{\mathcal{B}} \setminus a_i\},  a_i \neq a_k$
\sameer{what does this mean (formally)?}. \matt{I don't think this is the right formalization.  I think you want something like a function $f(q, a)$ that says where $a$ is an answer to $q$ (or $f(q) = a$, or something; there are lots of ways to define this).  What if $a_i$ and $a_k$ are paraphrases of each other?}\dheeru{wouldn't saying there is an injective mapping between the question and answer space be sufficient? because if $a_i$ and $a_k$ are paraphrases $q_i$ can match with two items in answer space}. In most of our discussion $n=2$, but this work can easily be extended to $n>2$ without loss of generality. 

To compute a real score for a given QA pair we employ compatibility function, $\psi$

% returns a score also referred to as exponentiated energy or potential for any given QA pair and is represented as $\psi(q_i, a_j) = \exp (d(q_i, a_j; \theta)) = s_{ij}$. 
% The different ways to parameterize function $d$ and to construct bundles are discussed in Section~\ref{sec:scores} and Section~\ref{sec:bundle} respectively.

\input{ACL2021/2-2-comp-scores}

\subsection{Existing methods}
Existing methods consider a single neighborhood either around question or answer. In this sub-section we elaborate on some of the existing single neighborhood models used in different NLP tasks.

\subsubsection{Maximum Likelihood Estimation}
Maximum likelihood training of question answering models entails independently maximizing the likelihood of the oracle answer over all possible answer candidates $\mathcal{A}$ for a given question.
\begin{equation}
    \begin{split}
       \mathcal{L(\theta)} &= \log \prod_{i=1}^n p(a_i|q_i) \\
       & = \sum_{i=1}^n \log \frac{\psi(q_i, a_i)}{\sum_{c \in \mathcal{A}} \psi(q_i, c)}
    \end{split}
\end{equation}

\subsubsection{Maximum Conditional Likelihood Estimation}
In cases with auto-regressive structured output, MLE is often replaced by a proxy loss maximum conditional likelihood (MCLE) which optimizes a lower-bound on the exact MLE. As length of the output reduces MCLE gets more closer to MLE hence can be effectively used to approximate short length answers. Intuitively, the global decision of choosing the right answer for all possible answers reduces to locally choosing the right word token from the entire vocabulary at each time step.
\begin{equation}
    \begin{split}
       \mathcal{L(\theta)} &= \log \prod_{i=1}^n p(a_i|q_i) \\
       &= \log \prod_{i=1}^n \prod_{t} p(a_i^t|a_i^{<t},q_i) \\
       &= \sum_{i=1}^n \sum_t \log \frac{\psi(a_i^t,q_i)}{\sum_{v \in V} \psi(a_i^v,q_i)}
    \end{split}
\end{equation}

\subsubsection{Unlikelihood}
A straightforward extension of likelihood training is to decrease the likelihood of negative answers in the neighbourhood of oracle answer for a given question by employing an unlikelihood objective~\cite{welleck2019neural} (UL).

\begin{equation}
    \begin{split}
        \mathcal{L}(\theta) = \sum_{i=1}^n \Big[ \log p(a_i|q_i) + \sum_{c \in \mathcal{A}_{B} \setminus a_i} \log(1 - p(c|q_i)) \Big]
    \end{split}
    \label{eq:ull}
\end{equation}

The second term in Eq.~\ref{eq:ull} helps provide additional signal to further reduce the likelihood of neighbouring negative answers, especially when the MLE loss starts to overfit at training~\cite{lewis2018generative}. 

\subsubsection{Contrastive Estimation}
Contrastive estimation~\cite{smith-eisner-2005-contrastive} (CE) was proposed for unsupervised structured prediction tasks like named entity recognition, where the probability mass from a perturbed un-grammatical (negative sample) input is moved to the oracle input summed up over all the tokens. 
A general CE formulation can be described as 

\begin{equation}
    \begin{split}
        \text{CE}(a_i, q_i) = \log p(a_i|q_i) &=  \\
        \log \frac{\psi(q_i, a_i)}{\sum\limits_{a_j \in \mathcal{A}_{\mathcal{B}}} {\sum\limits_{q_k \in \mathcal{Q}_{\mathcal{B}}}} \psi(q_k, a_j)}
    \end{split}
    \label{eq:ce_gen}
\end{equation}

 
We define \emph{single neighborhood} CE models as those that perturb and normalize over a single variable, question (input) or answer (output). Similarly, \emph{multiple neighborhood} CE models perturb both variables jointly and normalize over the combinatorial space of both variables.


This model can also be theorized as an energy based model which tries to push down energy of the oracle input-output pair over negative pairs. Energy based models often utilize noise contrastive estimation~\cite{gutmann2010noise} (NCE) which provides an efficient way of approximating the normalizer over a large space of candidates by learning a binary classifier, $BC$, that distinguishes gold pair from negative pairs. 

\begin{equation}
    \begin{split}
    \text{NCE}(a_i, q_i) = \log p(BC=1|a_i,q_i) + \\
    \sum_{(a_j, q_k) \in {\mathcal{A}_{\mathcal{B}} \times \mathcal{Q}_{\mathcal{B}}}} \log p(BC=0|a_j,q_k)
    \end{split}
    \label{eq:nce_gen}
\end{equation}

As we can see from Eq~\ref{eq:ce_gen} an Eq~\ref{eq:nce_gen} the neighbourhood does not take into consider false negative input-output pairs combinations, eg. ($q_j, a_j$), 

Since the number of input-output pair combinations are $O(n^2)$, in the number of instances in the bundle, $n$ which is generally quite small, we can easily employ CE instead of NCE. 

Unlikelihood training though easy to perform has two drawbacks. 
First, it independently minimizes the likelihood of the neighbourhood which means that the probability mass is moved from negative QA pairs but may not necessarily move to the positive pair unlike CE. Second, it does not allow capturing dependencies across multiple neighborhood i.e, question and answer neighbourhood jointly. 

  
% It uses a log-linear model which normalizes energies or compatibility scores over a neighbourhood of an input variable by perturbing it.


% Ideas similar to instance bundles have been explored in unlikelihood and (noise) contrastive estimation, however, they vary either question or answer but not both at the same time. We refer to these as single neighborhood models, as they vary (perturb) the neighborbood around a single variable, question or answer. 

% We propose using instance bundles to learn multi-neighborhood models that perturb question and answer neighborhood simultaneously, which allows the model to not only learn which answer contrastive answer is incorrect but also why is it incorrect by pairing the contrastive answer with the corresponding correct question. 

% Energy based models (EBM)~\cite{lecun2006tutorial} which learn an unnormalized compatibility score for a given QA pair provide an easy way to capture dependencies between a question and an answer. However, the compatibility score are unbounded and don't offer any probabilistic interpretation. Structured prediction tasks in NLP, often require a probablistic model to easily capture dependencies across structured inputs and outputs. To this end, contrastive estimation~\cite{smith-eisner-2005-contrastive} (CE) uses EBM style log-linear model that normalizes energies or compatibility scores over a neighbourhood of an input variable by perturbing it.
% All possible combinations of these neighbouring input samples and output labels (eg., part of speech tags) are considered for computing the normalization constant. Similar to energy based models, this learning method pushes the probability mass from neighbouring input-output pairs to the positive input-output pair. 

% The existing CE models consider token-level classification problems so have a fixed output space. We extend this approach to reading comprehension where the space of outputs increases linearly with length of context and exponentially with size of answer span. The computation of normalization constant over the entire output space becomes intractable. We use various sampling methods to approximate the output answer space and experiment with several normalization constants that offer different probabilistic interpretations.

% The CE based model contrastively considers a single neighborhood, question or answer at a time. We extend this framework and experiment with multiple neighborhood models which normalize across QA pairs in a bundle. We study their different probabilistic interpretations and compare them with single neighborhood models.

==> ACL2021/old_versions/3-model.tex <==
\section{Contrastive Estimation for Reading Comprehension}
\label{sec:model_old}

The unsupervised CE model sampled neighborhood around input and enumerated over all possible targets while performing sequence classification. However, in question answering the space of answers is much larger as number of targets are exponential in vocabulary size. This makes answer or question sampling procedure crucial for effective model learning. We discuss how to create bundles in Section~\ref{sec:bundle}


\begin{figure*}
\centering
\begin{subfigure}[b]{.24\textwidth}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=gray,text=black,minimum size=1cm]
  \tikzstyle{observed}=[circle,draw,fill=gray,text=white,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=5em]
  \tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]         (Q0) [left of=A0, xshift=-1cm]    {$q_0$};
  \node[question]         (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path[black, ultra thick] (Q0) edge              node {} (A0);
  \path[lightgray] (Q0) edge              node {} (A1);
  \node[plate, fit=(Q0)(Q1)(A0)(A1)] (containerq) {};
\end{tikzpicture}
\end{adjustbox}
\caption{Answer Conditional}
\label{fig:ans_cond}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.24\textwidth}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{observed}=[circle,draw,fill=gray,text=white,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=5em]
  \tikzstyle{factor}=[rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]         (Q0) [left of=A0, xshift=-1cm]    {$q_0$};
  \node[question]         (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path[black, ultra thick] (Q0) edge              node {} (A0);
  \path[lightgray] (Q1) edge              node {} (A0);
  \node[plate, fit=(Q0)(Q1)(A0)(A1)] (containerq) {};
\end{tikzpicture}
\end{adjustbox}
\caption{Question Conditional}
\label{fig:ques_cond}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.24\textwidth}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{observed}=[circle,draw,fill=gray,text=white,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=5em]
  \tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]

  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]           (Q0) [left of=A0, xshift=-1cm]      {$q_0$};
  \node[question]           (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path[black, ultra thick] (Q0) edge              node {} (A0);
  \path[lightgray] (Q0) edge              node {} (A1);
  \path[lightgray] (Q1) edge              node {} (A0);
  \path[lightgray] (Q1) edge              node {} (A1);
  \node[plate, fit=(Q0)(Q1)(A0)(A1)] (containerq) {};
\end{tikzpicture}
\end{adjustbox}
\caption{Multilabel}
\label{fig:multilabel}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.24\textwidth}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{observed}=[circle,draw,fill=gray,text=white,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=5em]
  \tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]         (Q0) [left of=A0, xshift=-1cm]    {$q_0$};
  \node[question]         (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path[black, ultra thick] (Q0) edge              node {} (A0);
  \path[lightgray] (Q0) edge              node {} (A1);
  \path[lightgray] (Q1) edge              node {} (A0);
  \node[plate, fit=(Q0)(Q1)(A0)(A1)] (containerq) {};
\end{tikzpicture}
\end{adjustbox}
\caption{Full partition}
\label{fig:full_part}
\end{subfigure}

% \hspace{1.5cm}
% \begin{subfigure}[t]{.2\textwidth}
% \centering
% \begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
%   \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
%   \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
%   \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
%   \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
%   \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=4em]

%   \node[ellipsis]           (C)                                 {};
%   \node[answer]           (A0) [right of=C, xshift=3cm]       {$q_0a_1$};
%   \node[answer]           (A1) [below of=A0, xshift=0cm]      {$q_1a_0$};
%   \node[question]           (Q0) [left of=A0, xshift=-1cm]      {$q_0a_0$};
%   \node[question]           (Q1) [left of=A1, xshift=-1cm]      {$q_1a_1$};
%   \path[blue] (Q0) edge              node {} (A0);
%   \path[red] (Q1) edge              node {} (A0);
%   \path[brown] (Q0) edge              node {} (A1);
%   \path[gray] (Q1) edge              node {} (A1);
%   \path[teal] (Q0) edge              node {} (Q1);
%   \path[olive] (A1) edge              node {} (A0);
%   \node[plate, fit=(Q0)(Q1)(A0)(A1)] (containerq) {};
% \end{tikzpicture}
% \caption{Joint(\dheeru{need to figure out how to show this correctly}}
% \label{fig:joint_cond}
% \end{subfigure}
\caption{Contrastive Estimation models}
\label{fig:multi_var}
\end{figure*}

\subsection{Single neighborhood models}
These models perturb a single variable (or neighborhood), i.e., question or answer while computing the normalization constant.


% \matt{You need to clarify what's going on here with sum vs. product and log vs. no log in all of these.  I would think that if you have a sum (e.g., in equations 6 and 7), you should have a log inside the sum.  Right?  Something is off in the math throughout this whole section, and this confusion is behind my question in section 3.3.2.  Might be easier to work this out over slack or in a meeting.}

\subsubsection{Answer Conditional}
This probabilistic model learns to push down the energy of positive answer, $a_i$ at the cost of its neighboring answers candidates for a given question, $q_i$. Figure~\ref{fig:ans_cond} shows a graphical instantiation of a bundle (with $n=2$, i.e., two QA pairs) for gold QA pair, $(q_0, a_0)$.


\begin{equation}
    \begin{split}
        \text{CE-AC}(\mathcal{B}) = \sum_{i=1}^n \log \frac{\psi(q_i, a_i)}{\sum_{a_j \in \mathcal{A}_\mathcal{B}} \psi(q_i, a_j)}
    \end{split}
    \label{eq:ans_cond}
\end{equation}

Since compatibility scores are exponentiated, this can be seen as a softmax that move the probability mass from positive to negative QA pairs.


\subsubsection{Question Conditional}
This model computes the normalization constant  over the question neighborhood for a fixed answer. Learning from different related questions encourages richer encoded representations. Figure~\ref{fig:ques_cond} shows a graphical instantiation of this normalizer.
\begin{equation}
    \begin{split}
       \text{CE-QC}(\mathcal{B}) = \sum_{i=1}^n \log \frac{\psi(q_i, a_i)}{\sum_{q_j \in \mathcal{Q}_{\mathcal{B}}} \psi(q_j, a_i)}
    \end{split}
    \label{eq:ques_cond}
\end{equation}



% \matt{Why not $\frac{\psi(q_i, a_i)}{\sum_{j \in |\mathcal{N}(a_i)|} \psi(q_i, a_j) + \sum_{j \in |\mathcal{N}(q_i)|} \psi(q_j, a_i)}$?  Oh, you have that in 3.2.1.  I don't really get the distinction you're making between section 3.1 and section 3.2, because this one meets the definition you have at the beginning of 3.2. }
% \dheeru{I was thinking of this as sum of two single neighbourhood and not really the cross product (in the normalizer) but on second thought you are right it is probably a simple way to do multiple neighborhood}

\subsection{Multiple neighbourhood models}
These models consider all possible combinations of questions,  $\mathcal{Q}_{\mathcal{B}}$ and answers, $\mathcal{A}_{\mathcal{B}}$ in a bundle for normalization, unlike single neighborhood models which only look at $\mathcal{A}_{\mathcal{B}}$ or $\mathcal{Q}_{\mathcal{B}}$ at a point in time.



\subsubsection{Two Way}
Similar to QAinfomax~\cite{yeh2019qainfomax}, this formulation is a mixture-of-experts~\cite{jacobs1991adaptive} style linear combination of answer and question conditionals. It tries to independently increase the likelihood over both question ans answer neighbourhoods.
\begin{equation}
    \begin{split}
       \text{CE-TW}(\mathcal{B}) = \sum_{i=1}^n \lambda_1 \log \frac{\psi(q_i, a_i)}{\sum_{a_j \in \mathcal{A}_\mathcal{B}} \psi(q_i, a_j)} + \\
       \lambda_2 \log \frac{\psi(q_i, a_i)}{\sum_{q_j \in \mathcal{Q}_\mathcal{B}} \psi(q_j, a_i)}
    \end{split}
    \label{eq:two_way_cond}
\end{equation}

\subsubsection{Multi Label}
In this model the likelihood of all gold QA pairs is maximized at the same time, similar to multi-label classification. This model can, unfortunately, increase the probability mass of a positive QA pair at the cost of another positive QA pair in the bundle.
\begin{equation}
    \begin{split}
       \text{CE-ML}(\mathcal{B}) = \sum_{i=1}^n \log \frac{\psi(q_i, a_i)}{\sum\limits_{\substack{q_j \in \mathcal{Q}_{\mathcal{B}}, \\ a_k \in \mathcal{A}_{\mathcal{B}}}} \psi(q_j, a_k)}
    \end{split}
    \label{eq:multilabel}
\end{equation}



% \matt{If I'm understanding the math right, this formula is wrong.  Shouldn't you have more than one term in the numerator?} \dheeru{ for n = 2 it will become $\frac{\psi(q_i,a_i)\psi(q_j,a_j)}{Z^2}$, its independently increasing lik. of each label, did I misunderstand something?}

\subsubsection{Joint}
We experiment with a well known alternative to multi-label classification, that entails expanding the label set such that each multi-label assignment becomes a new class label, known as a power-set label classification~\cite{zhang2007ml}. We perform this for only $n=2$ because the output space increase with $n$ as $O(n^2)$.
Let $s_{ij}$ be the compatibility score $\psi(q_i, a_j)$ then for $n=2$, the CE objective can be defined as

\begin{equation}
    \begin{split}
        \text{CE-JT}(\mathcal{B}) &=  \\
        \frac{s_{00} s_{11}}{s_{00} s_{11} + s_{00} s_{01} + s_{00} s_{10} + s_{01} s_{10} + s_{01} s_{11} + s_{10} s_{11}}
    \end{split}
\label{eq:joint}
\end{equation}


\begin{lemma}
The CE-ML objective is a lower bound on CE-JT objective. 
\end{lemma}
\begin{proof}
The CE-ML objective for independently aligning the right question-answer pair is 
\begin{equation}
    \begin{split}
        \exp(\text{CE-ML}(\mathcal{B})) &= \frac{s_{00}s_{11}}{(s_{00} + s_{11} + s_{10} + s_{01})^2} \\
        &= \frac{s_{00} s_{11}}{\splitfrac{2(s_{00} s_{11} + s_{00} s_{01} + s_{00} s_{10} \strut}
        {\splitfrac{{} + s_{01} s_{10} + s_{01} s_{11} + s_{10} s_{11}) } {\splitfrac{+ s_{00}^2 + s_{01}^2 + s_{10}^2 + s_{11}^2}{}}}} \\
    \end{split}
\label{eq:lemma}
\end{equation}

 $s_{00}^2 + s_{01}^2 + s_{10}^2 + s_{11}^2$ is a positive number. The denominator in Eq.~\ref{eq:lemma} is approximately equal to twice the denominator of Eq.~\ref{eq:joint}. This makes the gradient update for the positive pairs in case of joint model larger than that of multi label classifer.
\end{proof}

\subsubsection{Full Partition}
Based on the construction of bundles, each answer in $\mathcal{B_A}$ can only be correctly aligned with a single question in $\mathcal{B_Q}$. This allows for a formulation that increases likelihood of a oracle QA pair at the cost of all possible negative QA pairs only (which can be easily determined by the injective assumption on which instance bundles are built).
\begin{equation}
    \begin{split}
       \text{CE-FP}(\mathcal{B}) = \sum_{i=1}^n \log \frac{\psi(q_i, a_i)}{\sum\limits_{\substack{q_j \in \mathcal{Q}_{\mathcal{B}}, \\ a_k \in \mathcal{A}_{\mathcal{B}}, \\ j \neq k}} \psi(q_j, a_k)}
    \end{split}
    \label{eq:full_part}
\end{equation}

\subsection{Loss Interpolation}

On one hand, CE performs better than unsupervised expectation maximization~\cite{smith-eisner-2005-contrastive} by sampling from the neighbourhood around the input rather than the single input data point. However, it fails to do better than fully supervised MLE (or MCLE approximation) which increases the likelihood of oracle answer output over all possible answer candidates and not just the set of contrastive answers. 

On the other hand, MCLE can be sensitive to local probabilities of a sequence while CE considers the likelihood of entire sequence when learning the model providing a global perspective, especially when answer candidates are quite similar. Also, CE doesn't ensure conformity to local structure (for eg., deciding the correct length of answer) unlike MLE. 

For this reason, similar to unlikelihood training we use a combination of MLE and CE to get the benefits of MLE's local normalization and CE's global regularization.

\begin{equation}
    \mathcal{L} = \alpha_1 \mathcal{L}_{MCLE} + \alpha_2 \mathcal{L}_{CE}
\end{equation}




==> ACL2021/old_versions/introduction-old.tex <==
\section{Introduction}
The ease of training with assumption that data is sampled from an independent and identical distribution has allowed deep networks to effectively train with large reading comprehension datasets. However, this assumption can cause the learner to ignore distinguishing cues~\cite{dietterich1997solving} between related or minimally different~\cite{gardner-etal-2020-evaluating} questions associated with a given context, resulting in inconsistent model learning ~\cite{asai-hajishirzi-2020-logic,jia2017adversarial}. 
% To alleviate this problem, often various data augmentation~\cite{jiang2019avoiding,xie2020unsupervised} schemes are proposed to bridge gaps in learning.
In dataset like ROPES, where the ideology of collecting pairs of minimally different questions is taken to its extreme, we see that the baseline model performance is close to random~\cite{lin2019reasoning}. We believe that this is because the model learns to answer related question independently when it should be learning distinguishing cues between the questions that result in different answers.

% \begin{figure}[t]
% \begin{frame}
% \begin{textblock}
%     \begin{exampleblock}{}
   
%     \end{exampleblock}
% \end{textblock}
% }
\begin{figure}[t]
\begin{minipage}[t]{\textwidth}
\begin{tikzpicture}
\node[draw,text width=7.5cm]  at (0, 0) {\textbf{Background:} Old age begins in the mid-60s and lasts until the end of life. Most people over 65 have retired from work, freeing up their time for hobbies, grandchildren, and other interests. Stamina, strength, reflex time, and the senses all decline during old age, and the number of brain cells decreases as well. The immune system becomes less efficient, increasing the risk of serious illnesses such as cancer and pneumonia. Diseases such as Alzheimer's disease that cause loss of mental function also become more common.  \\
\textbf{Situation:} Two friends named Jill and Jane met after many years and had a chat over a cup of tea. Jane was 70 years-old, while Jill was 55. They shared many stories.};
\end{tikzpicture}
\end{minipage}
\begin{minipage}[t]{\textwidth}
\vspace{0.1cm}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.5cm,thick]
  \tikzstyle{question}=[align=center]
  \tikzstyle{answer}=[align=center]
  \tikzstyle{plateq}=[ellipse,draw,fill=none,minimum height=6em]
  \tikzstyle{platea}=[ellipse,draw,fill=none,minimum height=6em]
  
  \node[answer]           (A0) []       {Jane};
  \node[answer]           (A1) [below of=A0, yshift=-1.5cm]      {Jill};
  \node[question]           (Q0) [left of=A0,xshift=-2.5cm]      {\small Which friend \\ \small was most \\ \small likely retired \\  \small from work?};
  \node[question]           (Q1) [left of=A1,xshift=-2.5cm]      {\small Which friend \\ \small was probably \\ \small still working?};
  \path (Q0) edge              node {} (A0)
             edge              node {} (A1);
  \path (Q1) edge              node {} (A0)
             edge              node {} (A1);
  \node[platea, fit=(A0)(A1)] (containera) [] {};
  \node[plateq, fit=(Q0)(Q1)] (containerq) [] {};
\end{tikzpicture}
\end{minipage}
\caption{Example of instance bundle from ROPES}
\label{fig:ropes_ex}
\end{figure}


%   \textbf{Question 1:} Which friend was most likely retired from work? \\
%   \textbf{Answer 1:} Jane\\
%   \\
%   \\
%   \textbf{Question 2:} 
%   \textbf{Answer 2:} Jill


Inspired by contrastive estimation~\cite{smith2005contrastive} for unsupervised and representation learning~\cite{hjelm2018learning}, we propose a supervised technique to train the model with an instance bundle. An \emph{instance bundle} is a set of related or minimally different question-answer(QA) pairs such that there is an injective mapping between all the unique questions and the answers in the bundle. This style of multi-instance learning allows model to capture characteristic features that are crucial towards consistent learning. Figure~\ref{fig:ropes_ex} shows an example bundle mined from ROPES dataset. 

Our proposed model is trained by employing an energy-based framework~\cite{lecun2006tutorial}, which learns a compatibility function, that take a QA pair as input and outputs an un-normalized score to measures the affinity between the inputs. The objective function tries to increase the score of gold QA pairs normalized over scores of all possible QA pairs. We extensively study the impact of the normalization group, i.e. the set of possible QA pairs considered, on the model performance. The energy based frameworks allows for a probabilistic interpretation over these groups, which act as regularizers.


% We formulate contrastive estimation as a factor graph containing edges that connect the questions and answers in an instance bundle and then increase the likelihood for the gold edges over all other edges, effectively redistributing probability mass from negative factors to gold factors. We experiment with various different factor graph formulations to understand their effectiveness on different datasets.

In the cases, where we do not have access to sets of related questions readily available, we propose methods based on top-k sampling, nucleus sampling and domain specific mining heuristics to create instance bundles.We study the effectiveness of these heuristics on a variety of datasets.


Finally, whenever possible, we automatically generate an instance bundle given a new question at test time and show that solving the question-answering alignment as a linear sum assignment (hard) can further improve the overall model performance.

% We show performance improvements on four datasets: ROPES, HotpotQA, DROP and Quoref. 

[Something about results]



==> ACL2021/old_versions/model-old.tex <==
\section{Model Formulation}
\label{sec:model_old}
Given a training instance bundle of related question-answer pairs, $\mathcal{B} = \{(q_0...q_n),(a_0...a_n)\}$, the goal is to learn a random variable, $Z_n$, that selects $n$ compatible question-answer pairs from $\mathcal{B}$. In other words, $Z_n$ learns to align the  answers ($\mathcal{B}_A$) compatible with questions ($\mathcal{B}_Q$) in bundle $\mathcal{B}$. In most of our experiments, $n=2$ but this work can easily be extended to $n>2$ without loss of generality. To model the interactions within a bundle, we learn a compatibility function, $\psi$ which return a positive score also referred to as energy or potential of any given QA pair. 

\subsection{Setup}
Maximum likelihood training of question answering models entails independently maximizing the likelihood of the answer for a given question. 
\begin{equation}
    \begin{split}
       \mathcal{L(\theta)} = \sum_{i \in [1,n]} p(a_i|q_i)
    \end{split}
\end{equation}



Following~\cite{tishby2000information} we propose, a structured regularizer which maximizes the mutual information, $\mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q)$

\begin{equation}
    \begin{split}
       \mathcal{L}(\theta) = \sum_{i \in [1,n]} p(a_i|q_i) + \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q)
    \end{split}
    \label{eq:regularizer}
\end{equation}

The first term (cross-entropy) in Eq.~\ref{eq:regularizer} captures local interactions between the question and the answer in the given QA pair, while the  second term captures global interaction between across questions and answers and $\mathcal{B}_Q$ and $\mathcal{B}_A$ respectively. We can further re-write this mutual information (Eq.~\ref{eq:mi1}) by introducing alignment variable $Z_n$ to express the interaction between $\mathcal{B}_A$ and $\mathcal{B}_Q$

\begin{equation}
    \begin{split}
     \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q;Z_n)  = \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q) - \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q|Z_n)
    \end{split}
    \label{eq:mi1}
\end{equation}

\begin{equation}
    \begin{split}
    \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q) =  \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q;Z_n) + \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q|Z_n) \\
    \geq \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q|Z_n)
    \end{split}
    \label{eq:mi2}
\end{equation}


\begin{equation}
    \begin{split}
    \mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q|Z_n) = H(Z_n) - \big[H(Z_n|\mathcal{B}_A) + \\ H(Z_n|\mathcal{B}_Q) + H(Z_n;\mathcal{B}_A; \mathcal{B}_Q)\big]
    \end{split}
    \label{eq:mi3}
\end{equation}



Based on Eq.~\ref{eq:mi2} and Eq.~\ref{eq:mi3} maximizing a lower-bound on $\mathcal{I}(\mathcal{B}_A; \mathcal{B}_Q)$ is equivalent to minimizing the joint entropy $ H(Z_n;\mathcal{B}_A; \mathcal{B}_Q)$.

Several works~\cite{oord2018representation,hjelm2018learning} have shown that contrastive estimation objective maximizes a lower bound on mutual information. In similar vein, we propose, contrastive estimation based objective to maximize the structured regularizer in Eq~\ref{eq:mi3}. In the next sections,

\subsection{Unlikelihood}
A straightforward way to establish interactions  between $\mathcal{B}_A$ and $\mathcal{B}_Q$ independently without the need of alignment variable is to employ unlikelihood objective~\cite{welleck2019neural}.

\begin{equation}
    \begin{split}
        \mathcal{L}(\theta) = \sum_{i \in [1,n]} p(a_i|q_i) + \sum_{c \in \mathcal{B}_A \setminus a_i} (1 - p(c|q_i))
    \end{split}
    \label{eq:ull}
\end{equation}

This second term in Eq.~\ref{eq:ull} focuses on reducing the likelihood of negative answers for a given question.

\subsection{Single variable single edge selection model}
In this formulation, our alignment variable $Z_1$ picks a single edge, $e_{ij}$ from the set of edges, $\mathcal{E} = \{e_{ij}\} \bigcup\limits_{\substack{k \in |\mathcal{B}_Q|, l \in |\mathcal{B}_A| \\ k \neq l}} e_{kl} $, for a gold QA pair $(q_i,a_j)$. Figure~\ref{fig:single_factor_graph} shows an instantiation of the graph with two QA pairs $(n=2)$ in the bundle for gold QA pair, $(q_0, a_0)$. The probability of the random variable $Z_1$ can be decomposed into product of factors, where each factor $\psi(q_i,a_j)$ is an exponentiated score $\exp (d(q_i, a_j; \theta)) = s_{ij}$ and the parameterization function $d$ is discussed in Section~\ref{sec:scores}.

\begin{equation}
    \begin{split}
        p(Z_1,\mathcal{B}_A,\mathcal{B}_Q ) \propto \psi(q_0, a_0) \psi(q_1, a_0) \psi(q_0, a_1)
    \end{split}
\end{equation}

The model is trained to increase the likelihood of the gold edge, i.e, $e_{00}$ over the other edges (Figure~\ref{fig:single_factor_graph}). 
We study three different normalizations or partition functions (Figure~\ref{fig:single_var}) that have different probabilistic interpretations and contrastive effects on the compatibility function.

\begin{figure}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{observed}=[circle,draw,fill=lightgray,text=black,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=none,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum width=4em]
  \tikzstyle{factor}=[rectangle,fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \tikzstyle{score}=[align=center]

  \node[ellipsis]           (C)                                 {};
  \node[observed]           (A0) [right of=C,xshift=5cm]       {$a_0$};
  \node[observed]           (Q0) [left of=A0]      {$q_0$};
  \node[observed]           (Q1) [left of=Q0,xshift=-0.8cm]    {$q_1$};
  \node[observed]           (A1) [left of=Q1]      {$a_1$};
  \node[latent]           (Z1) [right of=C,xshift=5cm,yshift=3.5cm]      {$Z_1$};
  \node[plate, fit=(Q0)(A0)] (containerq) {};
  \node[plate, fit=(Q1)(A1)] (containera) {};
  
  \node[factor]           (F1) [above of=A0, xshift=0cm,yshift=1.8cm]    {};
  \node[factor]           (F2) [above of=Q0, xshift=0.5cm,yshift=1.8cm]   {};
  \node[factor]           (F3) [above of=Q0, xshift=-0.7cm,yshift=1.9cm]   {};
  \path (Q0) edge              node {} (F1);
  \path (A0) edge              node {} (F1);
  \path (Q1) edge              node {} (F2);
  \path (A0) edge              node {} (F2);
  \path (Q0) edge              node {} (F3);
  \path (A1) edge              node {} (F3);
  \path (Z1) edge              node {} (F1);
  \path (Z1) edge              node {} (F2);
  \path (Z1) edge              node {} (F3);
  
  \node[score]    (S1) [below of=F1,yshift=1.5cm,xshift=0.8cm] {\small $\psi(q_0, a_0)$};
  \node[score]    (S2) [below of=F2,yshift=1.1cm,xshift=-0.1cm] {\small $\psi(q_1, a_0)$};
  \node[score]    (S3) [below of=F3,yshift=1.6cm,xshift=-0.9cm] {\small $\psi(q_0, a_1)$};
  
  \node[score]    (E1) [below of=Z1,yshift=0.6cm,xshift=0.3cm] {\small $e_{00}$};
  \node[score]    (E2) [below of=Z1,yshift=0.6cm,xshift=-0.35cm] {\small $e_{10}$};
  \node[score]    (E3) [below of=Z1,yshift=0.6cm,xshift=-1.1cm] {\small $e_{01}$};
\end{tikzpicture}
\caption{Single variable single edge selection}
\label{fig:single_factor_graph}
\end{figure}



\subsubsection{Answer Conditional}
This model normalizes the probability of $Z_1$ over a partition of possible answers as shown in Figure~\ref{fig:ans_cond}. The set of answers, $\mathcal{B}_A$ can be obtained by various heuristics which are discussed in Section~\ref{sec:bundle}.
In other words, to minimize the conditional entropy, $H(Z_1|\mathcal{B}_A)$ (Eq.~\ref{eq:mi3}) we need to maximize the joint distribution $p(Z_1,\mathcal{B}_A)$

\begin{equation}
    \begin{split}
     p(Z_1,\mathcal{B}_A) = \sum_{q \in \mathcal{B}_Q} p(Z_1|\mathcal{B}_A, q) p(\mathcal{B}_A|q) p(q)
    \end{split}
\end{equation}

For a given fixed question, $q_0$ (uniform question prior), the probability of alignment variable given a bundle, $p(Z_1=e_{00} | \cdot)$\footnote{For succinct notation we will refer to $ p(Z_1=e_{00} | \mathcal{B_A}, \mathcal{B_Q})$ as $p(Z_1=e_{00} | \cdot)$}, choosing the gold edge $e_{00}$ is described in Eq.~\ref{eq:ans_cond}

\begin{equation}
    \begin{split}
        p(Z_1=e_{00} | \cdot) = \frac{\psi(q_0, a_0)}{\sum_{j \in |\mathcal{B_A}|} \psi(q_0, a_j)}
    \end{split}
    \label{eq:ans_cond}
\end{equation}



Intuitively, this model increases the likelihood of the QA pair in numerator (Eq.~\ref{eq:ans_cond}) at the cost of QA pairs in the denominator. The gradients will try to decrease the likelihood of even the gold QA along with negative QA pairs in the normalizer, however, combined with the numerator it will overall increase the likelihood of gold QA pair.

\begin{equation}
    \begin{split}
        \frac{\delta \log p(Z_1=e_{00} | \cdot)}{\delta \theta} = (I[j=0] - p(a_j|q_0)) \frac{\delta d(q_0,a_j)}{\delta \theta}
    \end{split}
    \label{eq:ans_cond}
\end{equation}


\begin{figure*}
\begin{subfigure}[t]{.2\textwidth}
\centering
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=4em]
  \tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]

  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]         (Q0) [left of=A0, xshift=-1cm]    {$q_0$};
  \node[latent]           (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path (Q0) edge              node {} (A0)
             edge              node {} (A1);
  \node[plate, fit=(Q0)(Q1)] (containerq) {};
  \node[plate, fit=(A0)(A1)] (containera) {};
\end{tikzpicture}
\caption{Answer Conditional}
\label{fig:ans_cond}
\end{subfigure}
\hspace{1.5cm}
\begin{subfigure}[t]{.2\textwidth}
\centering
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=4em]
  \tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]

  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[latent]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]           (Q0) [left of=A0, xshift=-1cm]      {$q_0$};
  \node[question]           (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path (Q0) edge              node {} (A0);
  \path (Q1) edge              node {} (A0);
  \node[plate, fit=(Q0)(Q1)] (containerq) {};
  \node[plate, fit=(A0)(A1)] (containera) {};
\end{tikzpicture}
\caption{Question Conditional}
\label{fig:ques_cond}
\end{subfigure}
\hspace{1.5cm}
\begin{subfigure}[t]{.2\textwidth}
\centering
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{question}=[circle,draw,fill=teal,text=white,minimum size=1cm]
  \tikzstyle{answer}=[circle,draw,fill=olive,text=white,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=white,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum height=8em, minimum width=4em]

  \node[ellipsis]           (C)                                 {};
  \node[answer]           (A0) [right of=C, xshift=3cm]       {$a_0$};
  \node[answer]           (A1) [below of=A0, xshift=0cm]      {$a_1$};
  \node[question]           (Q0) [left of=A0, xshift=-1cm]      {$q_0$};
  \node[question]           (Q1) [left of=A1, xshift=-1cm]      {$q_1$};
  \path (Q0) edge              node {} (A0);
  \path (Q1) edge              node {} (A0);
  \path (Q0) edge              node {} (A1);
%   \draw[dashed, -, inner sep=0pt] (Q1) -- (A1);
  \node[plate, fit=(Q0)(Q1)] (containerq) {};
  \node[plate, fit=(A0)(A1)] (containera) {};
\end{tikzpicture}
\caption{Full Conditional}
\label{fig:two_way_cond}
\end{subfigure}
\caption{Single edge selection}
\label{fig:single_var}
\end{figure*}


\subsubsection{Question Conditional}
Similar to answer conditional, we minimize the entropy $H(Z_1|\mathcal{B}_Q)$ by increasing the probability of edge $e_{00}$ normalized over a partition of contrastive questions as shown in Figure~\ref{fig:ques_cond}. The set of questions, $\mathcal{B}_Q$ can be obtained by various heuristics which are discussed in Section~\ref{sec:bundle}.

\begin{equation}
    \begin{split}
         p(Z_1=e_{00} | \cdot) = \frac{\psi(q_0, a_0)}{\sum_{j \in |\mathcal{B_Q}|} \psi(q_j, a_0)}
    \end{split}
\end{equation}

\dheeru{TODO: some intuition}

% \matt{This equation is identical to the question conditional equation. Something is off here.}
% \dheeru{oops copy error}
\subsubsection{Full partition}
This formulation combines the contrastive effects of both answer and question conditionals (Figure ~\ref{fig:two_way_cond}) by minimizing the joint entropy $H(Z_1, \mathcal{B}_Q, \mathcal{B}_A)$ (Eq.~\ref{eq:mi3}) .or maximizing the joint probability $p(Z_1, \mathcal{B}_Q, \mathcal{B}_A)$


\begin{equation}
    \begin{split}
     p(Z_1,\mathcal{B}_A, \mathcal{B}_Q) = p(Z_1|\mathcal{B}_A, \mathcal{B}_Q) p(\mathcal{B}_A,\mathcal{B}_Q)
    \end{split}
\end{equation}
The partition function for computeing $p(Z_1|\mathcal{B}_A, \mathcal{B}_Q)$ considers all possible negative question-answer combinations instead of just contrastive questions or contrastive answers.  

\begin{equation}
    \begin{split}
        p(Z_1 = e_{00} | \cdot) = 
        \frac{\psi(q_0, a_0)}{\sum\limits_{\substack{j \in |\mathcal{B_Q}|, k \in |\mathcal{B_A}| \\ j \neq k}} \psi(q_j, a_k)}
    \end{split}
\end{equation}




\subsubsection{Two-way}
Similar to QAinfomax~\cite{yeh2019qainfomax}, this formulation is a mixture-of-experts~\cite{jacobs1991adaptive} style linear combination of answer and question conditionals. It tries to independently increase the likelihood of both to simultaneously.

\begin{equation}
    \begin{split}
         p(Z_1=e_{00} | \cdot) \propto \lambda_1 \frac{\psi(q_0, a_0)}{\sum_{j \in |\mathcal{B_Q}|} \psi(q_j, a_0)} + \\
         \lambda_2\frac{\psi(q_0, a_0)}{\sum_{j \in |\mathcal{B_A}|} \psi(q_0, a_j)}
    \end{split}
\end{equation}




\subsection{Single variable multiple edge selection model}
This can be viewed as a multi-label classification model where the likelihood of multiple gold QA pairs 
is maximized at the same time. However, as the number of gold QA pairs increase the descending effects on gradients from the normalizer may start to balance out the ascending effects from the numerator. Intuitively, we treat the two gold QA pairs (Figure~\ref{fig:multiclass}) independent of each other while learning the random variable $Z_2$

\begin{equation}
    \begin{split}
        p(Z_2 = (e_{00}, e_{11}) | \cdot) = p(Z_1 = e_{00} | \cdot) p(Z_1 = e_{11} | \cdot) \\
        = \frac{\psi(q_0,a_0)}{\sum\limits_{\substack{j \in |\mathcal{B_Q}|, k \in |\mathcal{B_A}|}} \psi(q_j, a_k)} 
        \frac{\psi(q_1,a_1)}{\sum\limits_{\substack{j \in |\mathcal{B_Q}|, k \in |\mathcal{B_A}|}} \psi(q_j, a_k)} \\
    \end{split}
\end{equation}

\begin{figure}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{observed}=[circle,draw,fill=lightgray,text=black,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=none,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum width=4em]
  \tikzstyle{factor}=[rectangle,fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \tikzstyle{score}=[align=center]

  \node[ellipsis]           (C)                                 {};
  \node[observed]           (A0) [right of=C]       {$a_1$};
  \node[observed]           (Q0) [left of=A0]      {$q_1$};
  \node[observed]           (Q1) [left of=Q0,xshift=-1cm]    {$q_0$};
  \node[observed]           (A1) [left of=Q1]      {$a_0$};
  \node[latent]             (Zm) [above of=Q0, xshift=-1.2cm, yshift=1.8cm]      {$Z_2$};
  \node[plate, fit=(Q0)(A0)] (containerq) {};
  \node[plate, fit=(A1)(Q1)] (containera)[] {};
  
  \node[factor]           (F1) [above of=Q1, xshift=-0.8cm,yshift=1.5cm]    {};
  \node[factor]           (F2) [above of=A0, xshift=-0.8cm,yshift=1.5cm]   {};
  \node[factor]           (F3) [above of=Q1, xshift=0cm,yshift=1.5cm]   {};
  \node[factor]           (F4) [above of=Q0, xshift=0cm,yshift=1.5cm]    {};
  \path (Q1) edge              node {} (F1);
  \path (A1) edge              node {} (F1);
  \path (Q0) edge              node {} (F2);
  \path (A0) edge              node {} (F2);
  \path (A1) edge              node {} (F3);
  \path (Q0) edge              node {} (F3);
  \path (Q1) edge              node {} (F4);
  \path (A0) edge              node {} (F4);
  \path (Zm) edge              node {} (F1);
  \path (Zm) edge              node {} (F2);
  \path (Zm) edge              node {} (F3);
  \path (Zm) edge              node {} (F4);
  
  \node[score]    (S1) [above of=F1,yshift=-1.5cm,xshift=-0.6cm] {\small $\psi(q_0,a_0)$};
  \node[score]    (S2) [above of=F2,yshift=-1.5cm,xshift=0.7cm] {\small $\psi(q_1,a_1)$};
  \node[score]    (S3) [above of=F3,yshift=-1.5cm,xshift=0.7cm] {\small $\psi(q_1,a_0)$};
  \node[score]    (S4) [above of=F4,yshift=-1.5cm,xshift=-0.65cm] {\small $\psi(q_0,a_1)$};
  \node[score]    (E1) [above of=S1,yshift=-0.7cm,xshift=1.4cm] {\small $e_{00}$};
  \node[score]    (E2) [above of=S2,yshift=-0.7cm,xshift=-1.4cm] {\small $e_{10}$};
  \node[score]    (E3) [above of=S3,yshift=-0.8cm,xshift=1.1cm] {\small $e_{01}$};
  \node[score]    (E4) [above of=S4,yshift=-0.8cm,xshift=-0.9cm] {\small $e_{11}$};
\end{tikzpicture}
\caption{Single variable multi edge selection}
\label{fig:multiclass}
\end{figure}


\subsection{Multi variate multiple edge selection model}
In this formulation the alignment variable, $Z_n$ learns to pick, $n = min(|\mathcal{B}_Q|, |\mathcal{B}_A|)$ edges jointly in the graph  from the set of edges  $\mathcal{E} = \{\{e_{ij}\} \bigcup\limits_{\substack{k \in |\mathcal{B}_Q|, l \in |\mathcal{B}_A|}} e_{kl} \}$. Let $s_{ij}$ be the compatibility score $\psi(q_i, a_j)$.

\begin{equation}
    \begin{split}
        p(Z_n) \propto \prod\limits_{\substack{i \in |\mathcal{B}_A|, \\ j \in |\mathcal{B}_Q|}}  s_{ij}
    \end{split}
\label{eq:multi}
\end{equation}



Figure~\ref{fig:multi_variable} shows an instantiation of this model with two QA pairs. The partition function normalizes over all possible pairwise $(n=2)$ combinations of edges ($\Perm{|\mathcal{E}|}{2}$).
% \begin{equation}
%     \begin{split}
%         p(Z_m = (e_1,..e_m) = \\
%         \frac{\prod_i^m s_i}{\sum\limits_{\substack{j_1 \in [1,m], \\ j_2 \in [2, m] \\ ...\\ j_{m} \in [m-1, m] }} s_{j_1} s_{j_2}...s_{j_m}}
%     \end{split}
% \label{eq:multi}
% \end{equation}
The model objective is to increase the probability of picking the gold edge combination.
\begin{equation}
    \begin{split}
        p(Z_2 = (e_{00},e_{11}))  &=\\
        \frac{s_{00} s_{11}}{s_{00} s_{11} + s_{00} s_{01} + s_{00} s_{10} + s_{01} s_{10} + s_{01} s_{11} + s_{10} s_{11}}
    \end{split}
\label{eq:multi_ex}
\end{equation}

\begin{lemma}
The probability of selecting each edge independently is a lower bound on selecting $n$ edges jointly. 
\end{lemma}

\begin{proof}
If edges $e_{00}$ and $e_{1}$ are chosen independently, 
\begin{equation}
    \begin{split}
        p(Z_2 = (e_{00},e_{11})) &= \frac{s_{00} s_{11}}{(s_1 + s_2 + s_3 + s_4)^2} \\
        &= \frac{s_{00} s_{11}}{\splitfrac{2(s_{00} s_{11} + s_{00} s_{01} + s_{00} s_{10} \strut}
        {\splitfrac{{} + s_{01} s_{10} + s_{01} s_{11} + s_{10} s_{11}) } {\splitfrac{+ s_{00}^2 + s_{01}^2 + s_{10}^2 + s_{11}^2}{}}}} \\
    \end{split}
\label{eq:joint}
\end{equation}

 $s_{00}^2 + s_{01}^2 + s_{10}^2 + s_{11}^2$ is a positive number. The denominator in Eq.~\ref{eq:joint} is approximately equal to twice the denominator of Eq.~\ref{eq:multi_ex}, making the the distribution in Eq.~\ref{eq:joint} more peaky.
\end{proof}



\dheeru{TODO: generalize to n pairs}

\begin{figure}
\begin{tikzpicture}[-,>={stealth[black]},node distance=1.6cm,thick]
  \tikzstyle{observed}=[circle,draw,fill=lightgray,text=black,minimum size=1cm]
  \tikzstyle{latent}=[circle,draw,fill=none,text=black,minimum size=1cm]
  \tikzstyle{ellipsis}=[circle,fill=none,text=black,minimum size=1cm]
  \tikzstyle{plate}=[rectangle,draw,fill=none,minimum width=4em]
  \tikzstyle{factor}=[rectangle,fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
  \tikzstyle{score}=[align=center]

  \node[ellipsis]           (C)                                 {};
  \node[observed]           (A0) [right of=C]       {$a_1$};
  \node[observed]           (Q0) [left of=A0]      {$q_1$};
  \node[observed]           (Q1) [left of=Q0,xshift=-1cm]    {$q_0$};
  \node[observed]           (A1) [left of=Q1]      {$a_0$};
  \node[latent]             (Zm) [above of=Q0, xshift=-1.2cm, yshift=4cm]      {$Z_2$};
  \node[plate, fit=(Q0)(A0)] (containerq) {};
  \node[plate, fit=(A1)(Q1)] (containera)[] {};
  
  \node[factor]           (F1) [above of=Q1, xshift=-1.5cm,yshift=1.5cm]    {};
  \node[factor]           (F2) [above of=A0, xshift=-0.1cm,yshift=1.5cm]   {};
  \node[factor]           (F3) [above of=Q1, xshift=0cm,yshift=1.5cm]   {};
  \node[factor]           (F4) [above of=A0, xshift=-1.7cm,yshift=1.5cm]    {};
  
  \node[factor]           (F5) [above of=F1, xshift=-0.5cm,yshift=1.5cm]    {};
  \node[factor]           (F6) [right of=F5, xshift=1.2cm]   {};
  \node[factor]           (F7) [right of=F6, xshift=1.5cm]  {};
  \node[factor]           (F8) [right of=F7, xshift=1.8cm]    {};
  \node[factor]           (F9) [right of=F8, xshift=1cm] {};
  \node[factor]           (F10) [right of=F9, xshift=1cm]    {};
  \path (Q1) edge              node {} (F1);
  \path (A1) edge              node {} (F1);
  \path (Q0) edge              node {} (F2);
  \path (A0) edge              node {} (F2);
  \path (A1) edge              node {} (F3);
  \path (Q0) edge              node {} (F3);
  \path (Q1) edge              node {} (F4);
  \path (A0) edge              node {} (F4);
  \path (Zm) edge              node {} (F5);
  \path (Zm) edge              node {} (F6);
  \path (Zm) edge              node {} (F7);
  \path (Zm) edge              node {} (F8);
  \path (Zm) edge              node {} (F9);
  \path (Zm) edge              node {} (F10);
  
  \path (F1) edge [blue]      node {} (F5);
  \path (F3) edge [blue]      node {} (F5);
  \path (F1) edge [black]       node {} (F6);
  \path (F4) edge [black]       node {} (F6);
  \path (F1) edge [teal]       node {} (F7);
  \path (F2) edge [teal]       node {} (F7);
  \path (F4) edge [olive]       node {} (F8);
  \path (F3) edge [olive]       node {} (F8);
  \path (F2) edge [red]       node {} (F9);
  \path (F3) edge [red]       node {} (F9);
  \path (F2) edge [violet]       node {} (F10);
  \path (F4) edge [violet]       node {} (F10);

  
  \node[score]    (S1) [above of=F1,yshift=-1.5cm,xshift=-0.8cm] {\small $\psi(q_0,a_0)$};
  \node[score]    (S2) [above of=F2,yshift=-1.5cm,xshift=-0.6cm] {\small $\psi(q_1,a_1)$};
  \node[score]    (S3) [above of=F3,yshift=-1.5cm,xshift=-0.7cm] {\small $\psi(q_1,a_0)$};
  \node[score]    (S4) [above of=F4,yshift=-1.5cm,xshift=-0.65cm] {\small $\psi(q_0,a_1)$};
%   \node[score]    (E1) [above of=S1,yshift=-0.7cm,xshift=1.4cm] {\small $e_{00}$};
%   \node[score]    (E2) [above of=S2,yshift=-0.7cm,xshift=-1.4cm] {\small $e_{10}$};
%   \node[score]    (E3) [above of=S3,yshift=-0.8cm,xshift=1.1cm] {\small $e_{01}$};
%   \node[score]    (E4) [above of=S4,yshift=-0.8cm,xshift=-0.9cm] {\small $e_{11}$};
\end{tikzpicture}
\caption{Multi variable multi edge selection}
\label{fig:multi_variable}
\end{figure}


% \subsection{Connections to MLE}
% Maximum likelihood tries to maximize a lower bound on the mutual information between answer and question.
%  \begin{equation}
%     \begin{split}
%         I(A; Q) = \sum_{q \in Q}\sum_{a \in A} p(a, q) \log \frac{p(a, q)}{p(a)p(q)} \\
%         =  \sum_{q \in Q}\sum_{a \in A} p(a, q) \log \frac{p(a|q)}{p(a)} \\
%         \geq \sum_{q \in Q}\sum_{a \in A} p(a, q) \log p(a|q)
%         = KL(p(a|q)||p(a))
%     \end{split}
%     \label{eq:mle}
% \end{equation}

% For each question, MLE only considers a single answer. As shown in ~\cite{hjelm2018learning}, contrastive estimation allows sampling from a larger set of answer candidates aiding in computing better approximation to expectation.
% Following Donsker-Vardhan inequality for KL divergence, we can rewrite the above as.

% \begin{equation}
%     \begin{split}
%         I(A; Q) = KL(p(a|q) || p(a)) \\
%         \geq \mathbb{E}_{p(a|q)}[\psi(a,q)] - \log  \mathbb{E}_{p(a)}[\psi(a,q)] \\
%         \approx \mathbb{E}_{p(a|q)}[\psi(a,q)] - \log \mathbb{E}_{a \sim r(a|q)}[\psi(a,q)]
%     \end{split}
%     \label{eq:ce}
% \end{equation}

% Based on the bundling heuristic we sample answers from a distribution $r$ which takes question as input. 

% In case of a binary classification, maximizing the first term in Eq.~\ref{eq:ce} is generally sufficient as maximizing likelihood of gold class results in minimizing likelihood of incorrect class automatically. However, in case of high-dimensional output space modeling  $\log \mathbb{E}_{a \sim r(a|q)}[\psi(a,q)]$ to capture interactions between structured high-dimensional input, $Q$, and output, $A$ becomes more crucial to achieve a tighter bounder on mutual information.
